Re-evaluating Evaluation in Text Summarization

Automated evaluation metrics as a stand-in for manual evaluation are an essential part of the development of text-generation tasks such as text summarization. However, while the field has progressed, our standard metrics have not -- for nearly 20 years ROUGE has been the standard evaluation in most summarization papers. In this paper, we make an attempt to re-evaluate the evaluation method for text summarization: assessing the reliability of automatic metrics using top-scoring system outputs, both abstractive and extractive, on recently popular datasets for both system-level and summary-level evaluation settings. We find that conclusions about evaluation metrics on older datasets do not necessarily hold on modern datasets and systems.

==> conclusion.tex <==
\pg{conclusion to be written, perhaps after rest of our results come in}

\pfliu{I think we can highlight several potential applications of our HJ-datasets. For example: 0) improving meta evaluation by introduce more reference 1) recall (or F1) based factuality 2) design a learnable metric 3) combined with BLEURT, pretrianed + fine-tuned based metrics 4) meta$^2$ evaluation: diagnose the generalization ability of different metrics/or overfitting problems}

\pg{another thing that can come in conclusion: our recommendations for meta-evaluation papers, and papers introducing new metrics. (i) They should cover mutliple datasets, because we show that a metric that does well on one dataset could do poorly on others. (ii) They should cover system-level as well as summary-level settings, as metrics that do well in summary-level do not necessarily do well at system-level. }

Investigating the generalization ability of existing metrics to other datasets is also a crucial future research topic \gn{Move this to the ``future directions'' section in the conclusion}.
\pfliu{I think this could be one ``super-impressive'' observation. We also can highlight this in intro. }

==> datasets.tex <==
% \section{Preliminaries}

\subsection{Datasets}  

\noindent\textbf{TAC-2008, 2009}~\cite{tac2008,tac2009} are multi-document, multi-reference summarization datasets. Human judgements are available on for the system summaries submitted during the TAC 2008, TAC 2009 shared tasks.


\noindent\textbf{CNN/DailyMail (CNNDM)} \cite{hermann2015teaching} is a commonly used summarization dataset modified by \citet{nallapati2016abstractive}, which contains news articles and
associated highlights as summaries. We use the non-anonymized version. 

% \paragraph{XSum} \cite{narayan2018don} is a one-sentence summary dataset to answer the question ``What is the article about?''. All summaries are professionally written, typically by the authors of documents in this dataset. \mb{We must do HJ-free evaluation here}


==> experiment.tex <==
\section{Experiments}
\label{sec:experiments}
Motivated by the critical research question: \textit{are existing automatic metrics reliable}? We use the collected human judgments (based on 25 top-performing systems) to meta-evaluate current metrics from four diverse aspects, each measuring the ability of systems to: (1) rank \textit{all}-systems; (2) rank top-$k$ systems; (3) rank \textit{two}-systems; (4) rank system generated summaries. \pfliu{These four could be updated.} \mb{Is saying \textit{rank} the right thing to do here? Pearson's correlation checks for linearity as well.}\pfliu{Yes, let's ask for Graham's suggestions of these names.}


% \subsection{Exp-I: System-level Evaluation}
\subsection{Exp-I: Rank \textit{All}-Systems}
% \pfliu{Or ranking \textit{all}-Systems?}
\label{sec:williams_test}
%It's a commonly-used setting that using different metrics to 
% \mb{How about this: Automatic metrics serve the important purpose of ranking summarization systems and are widely used to create system leaderboards in NLP~\footnote{http://nlpprogress.com/english/summarization.html}. Thus, to meta-evaluate metrics, it is crucial to study if these system-level rankings correlate with human judgments, as done by~\citet{???}. Specifically, we ask two questions: }
Automatic metrics serve the important purpose of comparing summarization systems, and are widely used to determine where a new system ranks against existing state-of-the-art systems. Thus, in meta-evaluation studies, comparing automatic metrics against human judgements at a system-level is a commonly-used setting~\cite{bojar-etal-2016-wmt-results}.
We follow this setting by investigating how well each metric correlates with human judgment when ranking our collected $K=$25 systems.
% Then,
Specifically, we ask two questions:
% \pfliu{We should put ``system-level Pearson figure and william test figure as close as possible''. Additionally, can we also incorporate information obtained from william test to figure 1? For example, here is one of previous works' solution: ``correlations of metrics not significantly outperformed by any other for that language pair are highlighted in bold.''}
\paragraph{Can metrics reliably rank different systems?}
To answer this we observe the pearson correlation between different metrics and human judgments in Fig.~\ref{fig:pearson-mix}. \mb{Reminder to add system level ktau in appendix.} 
% \pg{suggestion: s/(1)/this/ as we havent numbered the question.} We find that 

\quad (1) most metrics have high correlations on the \texttt{TAC 2008} dataset but many suffer on \texttt{TAC 2009}, especially ROUGE based metrics. Notably, MoverScore and JS-2 are highly correlated with human judgements on \texttt{TAC 2009}. 

\quad (2) MoverScore, which was the best performing metric on \texttt{TAC 2008}, struggles on the \texttt{CNNDM mix} dataset.

\quad (3) ROUGE metrics consistently perform well on the collected \texttt{CNNDM} datasets.

\quad (4) Overall, metrics have lower correlations on \texttt{CNNDM Ext} dataset. The problem is much more severe for MoverScore and JS-2, which have moderate to high performance on all other datasets.

\paragraph{Are some metrics significantly better than others in ranking systems? }
% \pfliu{We should introduce ``System level Kendall’s tau correlation between metrics and human judgments across different datasets". Moreover, I think this is a common setting in which most previous metrics are evaluated, right?}

% \pfliu{Another thing should be noted: I try to re-read some old papers that usually calculate correlation based on at least two measures (Spearman, Pearson, Kendall), we should think about these questions: 1) should we introduce other measures 2) if yes, how to organize them, for example, if the observation of different correlation measure is consistent, we can keep one and put the other to the appendix. However, what if two measures say something different? We should highlight the differences and try to explain them. Also, we should re-organize the presentation of our figures.}

Since automated metrics calculated on the same data are not independent, 
% \pfliu{Despite this, I think we can not only focus on the results from William test. Based on the development of summarization's metrics, we first have 1) system-level Kendall’s tau correlation between metrics and human judgments 2) then we try to introduce William test to make more convincing results 3) then we have summary-level.  So, since a lot of previous works have done 1), we also should do it, just like previous works also present top-k results without reporting p-value. Nevertheless, we still can do it right. The good thing is we additionally have William Test as a bonus.} \mb{I don't think we'll be able to introduce williams' test if we start with kendall's tau. Moreover, we can have pearson correlation at the summary level instead of ktau (and move ktau to appendix). This will make our correlation measure consistent, comparable and we'll be able to use williams' test.} 
we must perform the Williams' test~\cite{williams-test} to establish if the difference in correlations between metrics is statistically significant~\cite{graham-baldwin-2014-testing}. In Fig. \ref{fig:williams_test} we report the p-values of Williams' test. 
% \paragraph{Result}
We find that 

\quad (1) MoverScore and JS-2 are significantly better than other metrics in correlating with human judgments on the \texttt{TAC} datasets.

\quad (2) On \texttt{CNNDM Abs} and \texttt{CNNDM Mix}, R-2 significantly outperforms all others whereas on \texttt{CNNDM Ext} none of the metrics show significant improvements over others.

\paragraph{Takeaway}
These results suggest that there is no one-size-fits-all metric that can outperform others on all datasets, indicating the need of using different metrics for different datasets. e.g. MoverScore on \texttt{TAC 2008}, JS-2 on \texttt{TAC 2009} and R-2 on \texttt{CNNDM} datasets. Additionally, metrics run the risk of overfitting to existing datasets and may not generalize to new datasets.
% -dependent metric. \mb{I'm not sure about the part. Should we advocate for a dataset dependent metric?}\pg{A more conservative takeaway could be: "indicating the need for dataset-based metric selection, i.e., using a metric that is known to work well for the specific dataset being used."}
% \pg{In this takeaway, we could bring up that moverscore is reliable on TAC 2008/2009 (evidenced by high pearson r) but not on CNN/DM Mix and Ext, and this shows the risk of dangerous overfitting when introducing a new metric but only evaluating on only one dataset}
\begin{figure}
    \centering
    \subfloat{
    \label{fig:tac_8_topk}
    \includegraphics[width=\linewidth]{emnlp2020-templates/images/williams-pearson-cnndm-mix.pdf}
  }
  
  \subfloat{
    \label{fig:cnn_dm_abs_topk}
    \includegraphics[width=\linewidth]{emnlp2020-templates/images/williams-pearson-cnndm-ext-abs.pdf}
  }
    \caption{\label{fig:pearson-mix}System level Pearson correlation between automatic metrics and human judgments. Please see Sec.~\ref{sec:williams_test} for more details.}
    \pfliu{Let's ask for Graham's suggestions: should we merge these two figures into one? If not, we should do the same for Fig.4 and Fig.5. It seems a bit of a wast of space.}
\end{figure}

%=========================================================

\begin{figure*}[ht]
  \centering
  \subfloat[TAC 2008]{
    \label{fig:tac_8_william}
    \includegraphics[width=0.2075\linewidth]{emnlp2020-templates/images/williams_tac.png}
  }
  \subfloat[TAC 2009]{
    \label{fig:tac_9_william}
    \includegraphics[width=0.175\linewidth]{emnlp2020-templates/images/williams_tac09.png}
  }
  \subfloat[CNNDM Abs.]{
    \label{fig:cnn_dm_abs_william}
    \includegraphics[width=0.175\linewidth]{emnlp2020-templates/images/williams_cnn_abs.png}
  }
  \subfloat[CNNDM Ext.]{
    \label{fig:cnn_dm_ext_william}
    \includegraphics[width=0.175\linewidth]{emnlp2020-templates/images/williams_ext.png}
  }
  \subfloat[CNNDM Ext.\& Abs.]{
    \label{fig:cnn_dm_mix_william}
    \includegraphics[width=0.175\linewidth]{emnlp2020-templates/images/williams_cnn_mix.png}
  }

\caption{\label{fig:williams_test}p-value of Williams' Significance Test for the hypothesis ``Is the system on left (y-axis) significantly better than system on top (x-axis)". `BScore' refers to BERTScore and `MScore' refers to MoverScore. A dark green value in cell $(i, j)$ denotes metric $m_i$ has a significantly higher \textit{Pearson} correlation with human scores compared to metric $m_j$ (p-value $< 0.05$).\footnote{Dark Green cells with p-value $= 0.05$ have been rounded up} `-' in cell $(i, j)$ refers to the case when \textit{Pearson} correlation of $m_i$ with human scores is less that of $m_j$. Please see Sec.~\ref{sec:williams_test} for more details.
% \pfliu{If we don't aim to put TAC 2009 here, probably we can put it in appendix.}
\mb{Why does our footnote disappear?}
\pfliu{The text labels of heatmaps can be ``bold'' and a little bigger.}
% \aash{added appendix for tac09}
}
\end{figure*}












\begin{figure*}[ht]
  \centering
  \subfloat[TAC-2008]{
    \label{fig:tac_8_topk}
    \includegraphics[width=0.205\linewidth]{emnlp2020-templates/images/tac-8-topk.pdf}
  }
  \subfloat[TAC-2009]{
    \label{fig:xsum}
    \includegraphics[width=0.1725\linewidth]{emnlp2020-templates/images/tac-9-topk.pdf}
  }
  \subfloat[CNNDM Abs]{
    \label{fig:cnn_dm_abs_topk}
    \includegraphics[width=0.1725\linewidth]{emnlp2020-templates/images/cnn-dm-abs-topk.pdf}
  }
  \subfloat[CNNDM Ext]{
    \label{fig:cnn_dm_ext_topk}
    \includegraphics[width=0.1725\linewidth]{emnlp2020-templates/images/cnn-dm-ext-topk.pdf}
  }
  \subfloat[CNNDM Mix]{
    \label{fig:cnn_dm_mix_topk}
    \includegraphics[width=0.1725\linewidth]{emnlp2020-templates/images/cnn-dm-mix-topk.pdf}
  }

\caption{System level \textit{Pearson} correlation with human judgements on top-$k$ systems. Please see Sec.~\ref{sec:topk_human} for more details.
% \gn{The units of the x axis are not clear, what do ``low, medium, and high'' mean? Why are there different numbers for each?}
}
 \label{fig:top_k_human}
\end{figure*}


% \begin{figure*}[ht]
%   \centering
%   \subfloat[TAC-2008]{
%     \label{fig:tac_8_lmh}
%     \includegraphics[width=0.24\linewidth]{emnlp2020-templates/images/tac-8-lmh.pdf}
%   }
% %   \subfloat[TAC 2009 topk.]{
% %     \label{fig:xsum}
% %     \includegraphics[width=0.19\linewidth]{emnlp2020-templates/images/tac-9-lmh.pdf}
% %   }
%   \subfloat[CNNDM Abs]{
%     \label{fig:cnn_dm_abs_lmh}
%     \includegraphics[width=0.24\linewidth]{emnlp2020-templates/images/cnn-dm-abs-lmh.pdf}
%   }
%   \subfloat[CNNDM Ext]{
%     \label{fig:cnn_dm_ext_lmh}
%     \includegraphics[width=0.24\linewidth]{emnlp2020-templates/images/cnn-dm-ext-lmh.pdf}
%   }
%   \subfloat[CNNDM Mix]{
%     \label{fig:cnn_dm_mix_lmh}
%     \includegraphics[width=0.24\linewidth]{emnlp2020-templates/images/cnn-dm-mix-lmh.pdf}
%   }

% \caption{\label{fig:lmh_human}System level \textit{Pearson} correlation for low, medium and high quality systems (non-cumulative).\gn{Try to make the color scheme consistent with the bar charts. In the bar charts the colors are a little light, so you may want to make similar colors but darker for this plot.}\aash{remember to add the caveat about result signficance.}} 
% \end{figure*}


% In figure~\ref{fig:summ_level_human} we report the summary level correlations between different metrics and human judgements, for different datasets. 




%\subsection{Exp-II: Top-k System-level evaluation} % Scoring Top-k Systems
\subsection{Exp-II: Rank \textit{Topk}-Systems}
\label{sec:topk_human}
% \pfliu{If putting top-k, bottom-k is a too difficult thing, why not remove bottom k? Let's only focus on topk. And I also have seen the observations of bottom-k are not many. Another advantages of removing bottom-k are: 1) the whole story can be unified:(?)[a) rank k system b) rank top-k system c) rank two system d) rank summary; 2) we can save space for other experiments, for example, if we aim to introduce one more correlation metric from (spearman, pearson, ken).}
Most papers that propose a new state-of-the-art system, often use 
automatic metrics as a proxy to human judgments, to rank their proposed method against other top scoring systems. However, \textit{can metrics reliably quantify the improvements that one high quality system makes over other competitive systems?}

To answer this, instead of focusing on all of the collected systems, we evaluate the correlation between automatic metrics and human judgments in ranking the \textit{top-k} systems, where \textit{top-k} are chosen based on a system's mean human score (Eqn. \ref{eqn:human_score}).
% \paragraph{Augmenting more systems }
% To obtain statistically significant correlations \gn{You shouldn't aim to achieve statistically significant correlations, that's not the goal. The goal is to test a hypothesis in an appropriate way. It's not clear to me why this is the appropriate way to do so...}, we 
% follow~\citet{bert-score} and augment the collected systems by randomly sampling output summaries from the set of collected summaries for each document. This is done to generate 1000 additional synthetic systems. For \texttt{CNNDM Ext}, this leads to generating 11 systems that are even better than the current state-of-the-art \gn{Why? I don't understand this. Do you mean \emph{some} of the randomly sampled systems are better than the state of the art? If so, that's not super-interesting, because if I generate enough random results I'd eventually get a really good one. It's like the old ``monkeys on typewriters'' thing.}. 
% \quad (1) Top-k Systems (Cummulative): We partition all summarization systems into cumulative bins according to a system's mean human score (Eqn \ref{eqn:human_score}), each bin containing the \textit{top-k} systems for different values of $k$.
% \quad (2) Low / Medium / High Quality (Non-cummulative): We partition all summarization systems in 3 equal-sized bins sorted according to a system's mean human score (Eqn. \ref{eqn:human_score}) to categorize the systems intolow, medium and high quality based on their relative scoring. \aash{merging 4.2/4.3}
% \paragraph{Results}
\pfliu{Enumerate different observations using bullets with the same style.}
Our observations are presented in Fig.~\ref{fig:top_k_human}. We find that: 

\quad (1) as $k$ becomes smaller, metrics de-correlate with humans on the \texttt{TAC-2008} and \texttt{CNNDM Mix} datasets, even getting negative correlations for small values of $k$ (Fig. \ref{fig:tac_8_topk}, \ref{fig:cnn_dm_mix_topk}). 

\quad (2) Interestingly, SMS, R-2 and JS-2 \textit{improve} in performance as $k$ becomes smaller on \texttt{CNNDM Ext}. 

\quad (3) R-2 remains highly correlated with human judgements on \texttt{CNNDM Abs} for all values of $k$. However, it has negative correlations with human judgements on \texttt{TAC 2009} for $k < 50$.

% \quad (4) For non-cumulative setting, as systems become stronger, the correlation of automated metrics and human scores reduces and metrics correlate the best with humans for low quality systems. This trend is consistent across all datasets but is more severe on the \texttt{TAC-2008} dataset, where ROUGE metrics have a negative correlation with human scores for high quality systems. 

\paragraph{Takeaway }Metrics cannot reliably quantify the improvements made by one system over others, especially for the top few systems across all datasets. Some metrics, however, are well suited for some datasets, e.g. JS-2 and R-2 are reliable indicators of improvements on \texttt{TAC 2009} and \texttt{CNNDM Abs}.
\pfliu{Should we add a caveat of not reporting p-value}
% In addition to summary level, even at the system level meta-evaluations of metrics on the \texttt{TAC} datasets are no longer valid.
% Metrics are more reliable when quantifying improvements on low quality systems as compared to medium or high quality systems.

% \subsection{Exp-III: Scoring Systems of Varying Quality}
% \label{sec:quality_human}
% In Sec. \ref{sec:topk_human}, we analyzed the behavior of metrics on top scoring systems.
% In this experiment, we ask the question: \textit{are automated metrics more reliable when measuring the improvements in low quality, medium quality, or high quality systems?}
% We follow a similar strategy as Sec.~\ref{sec:topk_human} to generate 1000 systems in addition to the collected systems and partition them in 5 equal-sized bins according to a system's mean human score (Eqn. \ref{eqn:human_score}). For the \texttt{TAC-2008} dataset, we partition the systems into 3 equal-sized bins~\footnote{Since the TAC-2008 dataset has 58 systems, we could only use 3 bins to maintain statistical significance within each bin.}.
% \paragraph{Results}
% Our observations in Fig.~\ref{fig:lmh_human} reveal an interesting property of metrics - overall, as systems become stronger, the correlation of automated metics and human scores reduces. Indeed, metrics correlate the best with humans for low quality systems. This trend is consistent across all datasets.
% This problem is more severe on the \texttt{TAC-2008} dataset, where ROUGE metrics have a negative correlation with human scores for high quality systems. Please see Fig. \ref{fig:tac_9_lmh} in Sec. \ref{sec:tac_2009_obs} for corresponding results on the \texttt{TAC-2009} dataset.

% \paragraph{Takeaway }Metrics are more reliable when quantifying improvements on low quality systems as compared to medium or high quality systems.

% \subsection{Exp-IV: Significance testing using William's test}
% \label{sec:williams_test}
% In this experiment, we aim to establish if one metric is significantly better than others, on the whole scoring range, in terms of its correlation with human judgments. Since automated metrics calculated on the same data are not independent, we must perform The William's test~\cite{williams-test} to establish if the difference in correlations between metrics is statistically significant~\cite{graham-baldwin-2014-testing}. In Fig. \ref{fig:williams_test} we report the p-values of William's test. Please see Fig.~\ref{fig:tac09_williams} in Sec. \ref{sec:tac_2009_obs} for corresponding results on the \texttt{TAC 2009} dataset.
% For pearson's correlation values, please see Fig. \ref{fig:williams_pearson} in Sec.~\ref{sec:williams_pearson}
% % In figure(s) ?\pfliu{missing} \mb{Still thinking if we need to add the absolute value of pearson's correlation or not. Added to appendix for now.} we report the \textit{Pearson}correlation between metrics and humans on different datasets, and in figure \ref{fig:williams_test}, we report their corresponding p-values.

% \paragraph{Result}
% We find that on \texttt{CNNDM Ext}, none of the metrics significantly outperforms all others, while on \texttt{CNNDM Abs}, ROUGE-1 and ROUGE-2 are significantly better than others. On the other hand, on the \texttt{TAC-2008} dataset, MoverScore outperforms all others.

% \paragraph{Takeaway}
% These results suggest that there is no one-size-fits-all metric that can outperform others on all datasets. This highlights the importance of a dataset-dependent metric.
% % \pfliu{Usually, after we describe intuitive results, we also should discuss some insightful points. For example:``above results suggest that there is no one-size-fits-all metric that can outperform others on all datasets. This highlights the importance of a dataset-dependent metric.''}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.99\linewidth]{emnlp2020-templates/images/bootstrap.pdf}
%     \caption{\label{fig:bootstrap}F1-Scores with bootstrap resampling. Please see Sec. \ref{sec:bootstrap} for more details.}
% \end{figure}

%=========================================================
% \subsection{Exp-V: Pairwise System Ranking using Bootstrap Resampling}
\subsection{Exp-III: Rank $Two$-Systems}
% \subsection{Exp-IV: System Discrimination Ability}
\label{sec:bootstrap}


% \pfliu{Can we say another characteristic of rank 2-sys is we can not refer to correlation measures? (I mean we need use some correlation measure for rank k-sys)}


% \pfliu{For the motivation of rank 2-sys, we can also highlight the differences with rank k-sys (or someting that rank k-sysn can not do.). Then our story will be more coherent.}

Instead of of ranking a bunch of systems (Sec.~\ref{sec:williams_test}, ~\ref{sec:topk_human}) ranking $two$-systems aims to test the discriminative power of each metric, i.e., the degree to which one metric can capture statistically significant differences between two summarization systems.

% \pfliu{We might condense the following description.}

Specifically, in Sec.~\ref{sec:topk_human} we established that most metrics do not correlate well with human judgments when scoring current best-performing systems. However, often, we only care about measuring if one system is significantly better than another e.g., we might want to see if a new potential state-of-the-art system is better than the current best-performing system.
In this experiment, we analyze the reliability of metrics along this useful dimension: \textit{can metrics reliably say if one system is significantly better than another}?

Given two systems $Sys_1$ and $Sys_2$, one can compare the mean scores received by each system to establish which system is better. However, as a field matures, the differences in scores typically become smaller. In such scenarios, we must use a statistical significance test to claim with some confidence, if one system is better than another. For our use case, Paired Bootstrap Resampling is an ideal statistical test, since we have only 100 human-annotated outputs per system \cite{bootstrap_paper,dror-etal-2018-hitchhikers}.
% \pfliu{I added one more reference}.

Therefore, we take all $J \choose 2$ pairs of systems and compare their mean human score (Eqn. \ref{eqn:human_score}) using Paired Bootstrap Resampling. We assign a binary label $y_{true} = 1$ if $Sys_1$ is better than $Sys_2$ with 95\% confidence, and $y_{true} = 0$ for vice-versa~\footnote{We never obtain the case when the confidence of a prediction is less than 95\% ; we observe that both human judgements and metrics make confident predictions}. We treat this as the ground truth label of the pair $(Sys_1, Sys_2)$. This process is then repeated for all metrics, to get a ``prediction", $y_{pred}^m$ from each metric $m$ for the same $J \choose 2$ pairs. If $m$ is a good proxy for human judgments, the F-1 score between $y_{pred}^m$ and $y_{true}$ should be high. We calculate the weighted macro F-1 score for all metrics and view them in Fig. \ref{fig:bootstrap}.

We find that most metrics perform moderately well in this task; many achieve greater than 0.8 F-1. ROUGE-2 performs the best on \texttt{CNNDM Abs}, achieving an F-1 score of 0.96, while ROUGE-1 performs the best for \texttt{CNNDM Ext}. While on the \texttt{TAC} datasets, MoverScore achieves high F-1 scores, its performance is low on \texttt{CNNDM Ext}.

\paragraph{Takeaway } Automated metrics can often reliably predict if one system better than another. However, different metrics are better suited for different datasets and kinds of systems. For example, on the \texttt{CNNDM} dataset, we recommend using ROUGE-2 to compare abstractive systems and ROUGE-1 to compare extractive systems. While, on the TAC datasets, we recommend using MoverScore. \pfliu{These are interesting and I think they could be put in intro:observation section.}


\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{emnlp2020-templates/images/bootstrap.pdf}
    \caption{\label{fig:bootstrap}F1-Scores with bootstrap resampling. Please see Sec. \ref{sec:bootstrap} for more details.}
\end{figure}

%=========================================================
\subsection{Exp-IV: Rank Summaries}
\label{sec:summ_level_human}
% \mb{Can we change the first para to: In addition to ranking systems, real-world application scenarios also require metrics to reliably rank multiple summaries of a document. For example, top-scoring reinforcement learning based summarization systems~\cite{bohm2019better,zhong2020extractive} heavily rely on summary-level reward scores to guide the optimization process.}

In addition to ranking systems, real-world application scenarios also require metrics to reliably rank multiple summaries of a document. For example, top-scoring reinforcement learning based summarization systems~\cite{bohm2019better} and the current state-of-the-art extractive system~\cite{zhong2020extractive} heavily rely on summary-level reward scores to guide the optimization process.

In this experiment, we ask the question:
\textit{how well do different metrics perform at a summary-level, i.e. in ranking system summaries generated from the same document?}
% \textit{how well do different metrics rank the generated summaries of top-scoring systems on diverse datasets?} \pg{suggested rephrase for clarity: \textit{how well do different metrics perform at a summary-level, i.e. in ranking system summaries generated from the same document?}}
We use Eq.~\ref{eqn:summ_level_corr} to calculate Pearson's correlation between different metrics and human judgments for different datasets and collected system outputs.
%\subsection{Exp-II: Summary-level Evaluation} % Ranking Top Scoring Summaries
 \begin{figure}
    \centering
    % \includegraphics[width=0.99\linewidth]{emnlp2020-templates/images/exp/summ-level-1.pdf}
    \includegraphics[width=0.99\linewidth]{emnlp2020-templates/images/sum-level-pearson.pdf}
    \caption{\label{fig:summ_level_human}Summary level \textit{Pearson}'s correlation between metrics and human judgements across different datasets. Please see Sec~\ref{sec:summ_level_human} for more details.}
\end{figure}

% \pfliu{The following paragraph can be heavily compressed or even removed (put in related work HJ-free).}
% \citet{peyrard-2019-studying} study the correlation among different automatic metrics at the summary level 
% \pfliu{Currently, we motivate ``summary-level evaluation'' by using Peyrard's scoring range observation. It makes sense, however, we have some other choices that we can try to do it from the real-world scenario of summary-level evaluation. For example, 1) it could be the time you want to #only# compare two generated summaries from several diverse systems instead of two set of summaries; 2) it could be the time you want to design a summary-level reward function for RL-based abstractive summarization or even for matchSum (a summary-level SOTA extractive summarization system); In brief, we can explain why we conduct summary-level experiment using our newly-collected human judgment from its significance in real-world application; This two papers can be referred: 1) https://www.aclweb.org/anthology/D19-1307.pdf  2) https://www.aclweb.org/anthology/P18-1060.pdf} 
% and find that metrics disagree with each other in ranking the top-scoring summaries of each document. However, their meta-evaluation framework fails to address the useful question: \textit{do some metrics correlate with human judgments in ranking top scoring summaries?} In this experiment, we aim to fill this research gap by analyzing the correlations between metrics and humans, for summaries generated by current top-scoring systems, on modern datasets. 

\paragraph{Results}
Our observations are summarized in Fig.~\ref{fig:summ_level_human}. We find that:

\quad (1) As compared to semantic matching metrics, R-1, R-2 and R-L have lower correlations on the \texttt{TAC} datasets but are strong indicators of good summaries especially for extractive summaries on the \texttt{CNNDM} dataset.

\quad (2) Notably, BertScore, R-1 and R-L have \textit{negative} correlations on \texttt{TAC 2009} but perform moderately well on other datasets.

\quad (3) Previous meta-evaluation studies~\cite{chaganty2018price} conclude that automatic metrics tend to correlate well with humans at the system level but have poor correlations at the summary level. We find this observation to be consistent on our \texttt{CNNDM} human judgement dataset. One notable exception is MoverScore, which has a correlation of only 0.05 on \texttt{CNNDM Ext} at the system level but 0.66 at the summary level.

% \quad (1) Metrics have low correlations with human judgments at the summary level \pfliu{Can we introduce system-level experiments first since 1) it's more intuitive setting (also in line with the development of meta-evaluation history?) 2) once we introduce system-level first, we can easier compare summary-level and system-level and claim ``metrics'' have lower correlations at summary-level compared with system-level (the comparison is meaningful since existing work always claimed that ROUGE performs better at system-level compared with summary-level, here we can investigate if this conclusion holds true in CNNDM dataset and how other metrics perform in these two settings, in different datasets, for example, ``will MoverScore get a higher summary-level score compared with system-level setting on CNNDM?''. If we know: 1) a metric performs best at summary-level in a dataset A, 2) and the absolute value of the summary-level correlation (with human judgment) is pretty higher, for example higher than it system-level score, this is very uesful information since we can use this metric to design summary-level rewards function for reinforcement learning. In brief, based on the metric's summary-level performance and its comparison with system-level performance, we can searching for effective summary-level reward function for reinforcement learning.) } and particularly struggle to rank a mixture of extractive and abstractive summaries on the \texttt{CNNDM} dataset. The correlation with human scores on \texttt{(CNNDM Abs, CNNDM Ext)} datasets is higher than correlation on previous datasets. \gn{This is low, but it's actually \emph{higher} than TAC. What is the criterion for ``low''? Has something changed since ``TAC'' or are things relatively similar?} 

% \quad (2) Notably, a recently proposed metric, MoverScore, that achieves the best performance on the previous human judgment datasets (\texttt{TAC-2008, TAC-2009}), actually performs \emph{worst} on our newly-collected, \texttt{CNNDM Mix} datset.
% This suggests a significant gap between the efficacy of evaluation metrics on the older systems in the \texttt{TAC} dataset and our new benchmark.

\paragraph{Takeaway }Meta-evaluations of metrics on the old \texttt{TAC} datasets show significantly different trends than meta-evaluation on modern systems and datasets.
Moreover, some metrics may not generalize to different datasets e.g. BERTScore on \texttt{TAC 2009} vs others. This highlights the need for empirically testing the efficacy of different automatic metrics in ranking summaries on multiple datasets (e.g. a meta-evaluation benchmark like GLUE~\cite{wang2018glue}). Moreover, consistent with previous findings, most automatic metrics correlate better at the system level on the newly curated \texttt{CNNDM} dataset. However there are exceptions e.g. MoverScore on \texttt{CNNDM Ext}. This shows that even though some metrics might be good at ranking summaries, they may point in the wrong direction when ranking systems.

% \pfliu{This sentence could be useful: ``Since MoverScore is a newly proposed metric, which has achieved best result at summary-level setting of the TAC dataset (without system-level evaluation), it is easy to mislead researchers to blindly use it to rank systems. Therefore, our observation prevents them from going in a wrong direction.''}


% \gn{Not sure where this is shown? Could you clarify?}.
%=========================================================

% \subsection{Exp-VI: Effect of different properties of documents}
% \label{sec:properties}

% \subsubsection{Extractiveness}
% \mb{To be added to appendix}
% In addition to the scoring range, we also analyse the effect of three other properties on the correlation of evaluation metrics. All of these properties measure some form of \textit{extractiveness} of the source document-reference summary pair.

% \begin{enumerate}
%     \item \textbf{Abstractiveness} We define the \textit{abstractiveness} of a document as the percentage of tokens in the reference summary which are not present in the source document.
%     \item \textbf{Extractive fragment coverage \footnote{We simply refer to this as coverage}} \cite{grusky-etal-2018-newsroom} measures the percentage of words in the reference summary that are a part of any extractive fragment of the source document.
%     \item \textbf{Extractive fragment density \footnote{We simply refer to this as density}} \cite{grusky-etal-2018-newsroom} measures average length of the extractive fragment to which each word in the summary belongs.
% \end{enumerate}

% For all of the properties, we plot the kendall's tau correlations between different metrics on both Synth-Ext and Sota-Abs system outputs of the CNN/DailyMail dataset in figure \ref{fig:cnndm_properties}. 
% Here, each point is a document, y-axis measures the correlation and x-axis measures the respective property.

% Overall, we observe that as the extractiveness of the (document, reference) pair increases, the correlation among metrics increases.
% We find similar trends across different metric pairs and other datasets. \mb{Include all of the plots in the appendix}

% \begin{figure*}
% \begin{subfigure}{10em}
%   \centering
%   \includegraphics[width=10em]{emnlp2020-templates/images/cnn_dm_r2_rl_abstractiveness.png}
%   \caption{\label{fig:cnndm_ga_abs_ktau}Abstractiveness vs ktau}
% \end{subfigure}%
% \begin{subfigure}{10em}
%   \centering
%   \includegraphics[width=10em]{emnlp2020-templates/images/cnn_dm_r2_rl_coverage.png}
%   \caption{\label{fig:cnndm_ga_cov_ktau}Coverage vs ktau}
% \end{subfigure}
% \begin{subfigure}{10em}
%   \centering
%   \includegraphics[width=10em]{emnlp2020-templates/images/cnn_dm_r2_rl_density.png}
%   \caption{\label{fig:cnndm_ga_den_ktau}Density vs ktau}
% \end{subfigure}
% \begin{subfigure}{10em}
%   \centering
%   \includegraphics[width=10em]{emnlp2020-templates/images/cnn_dm_r2_rl_eos.png}
%   \caption{\label{fig:cnndm_ga_eos_ktau}Ease of Summarization vs ktau}
% \end{subfigure}
% \begin{subfigure}{10em}
%   \centering
%   \includegraphics[width=10em]{emnlp2020-templates/images/cnn_dm_abs_r2_rl_abstractiveness.png}
%   \caption{\label{fig:cnn_dm_abs_abs_ktau}Abstractiveness vs ktau}
% \end{subfigure}%
% \begin{subfigure}{10em}
%   \centering
%   \includegraphics[width=10em]{emnlp2020-templates/images/cnn_dm_abs_r2_rl_coverage.png}
%   \caption{\label{fig:cnn_dm_abs_cov_ktau}Coverage vs ktau}
% \end{subfigure}
% \begin{subfigure}{10em}
%   \centering
%   \includegraphics[width=10em]{emnlp2020-templates/images/cnn_dm_abs_r2_rl_density.png}
%   \caption{\label{fig:cnn_dm_abs_den_ktau}Density vs ktau}
% \end{subfigure}
% \begin{subfigure}{10em}
%   \centering
%   \includegraphics[width=10em]{emnlp2020-templates/images/cnn_dm_abs_r2_rl_eos.png}
%   \caption{\label{fig:cnn_dm_abs_eos_ktau}Ease of Summarization vs ktau}
% \end{subfigure}
% \caption{\label{fig:cnndm_properties}\textbf{Top}: The effect of various properties on correlations of metrics on the Synth-Ext extractive outputs on the CNN/DailyMail dataset.
% \textbf{Bottom}: The effect of various properties on correlations of metrics on the Sota-Abs outputs on the CNN/DailyMail dataset.
% In each plot, every point represents the kendall's tau correlation of Rouge-2 and Rouge-L on the document on the y-axis and the respective property on the x-axis. Overall we find that as extractiveness of a document increases, correlation between metrics increases on the Synth-Ext extractive system outputs but this trend vanishes for the Sota-Abs outputs. We also find that for both extractive and abstractive outputs, higher EoS leads to higher correlations. Please see section \ref{sec:exp1} for more details}
% \end{figure*}


% \subsubsection{Ease of summarization}
% \mb{to be added to appendix}
% We define \textit{ease of summarization} (EoS) of a document $d_i$ as the average of the maximum normalized score that all of it's system summaries received. i.e. 
% \begin{equation}
%     EoS(d_i) = \frac{1}{m} \sum_{j = 1}^m \max_{m_k} m_k(s_{ij})
% \end{equation}
% where $m_k$ is the normalized score on metric $k$ received by $j^{th}$ output summary of $d_i$. 

% The kendall's tau correlations for some representative metric pairs on the CNN/DailyMail dataset are plotted in figure \ref{fig:cnndm_properties}. We find similar trend across other metric pair and other datasets. Overall, we observe that as ease of summarization increases, correlations between metrics increases.



==> human_eval.tex <==
%\section{Human Evaluation Methodology}
%\section{Meta-evaluation with Human Judgement}

% \pfliu{It seems that we can make it a new section}
\section{Collection of Human Judgments}
\label{sec:human_collection}
We follow a 3-step process to collect human judgments:
% The process of collecting human judgments contains three steps:
(1) we \emph{collect} system-generated summaries on the most-commonly used summarization dataset, \texttt{CNNDM};  
(2) we \emph{select} representative test samples from \texttt{CNNDM} and 
(3) we manually \emph{evaluate} system-generated summaries of the above-selected test samples.

\subsection{System-Generated Summary Collection}
We collect the system-generated summaries from 25 top-scoring systems,\footnote{We contacted the authors of these systems to gather the corresponding outputs, including variants of the systems.} covering 10 extractive and 15 abstractive systems (Sec.~\ref{sec:system}) on the \texttt{CNNDM} dataset. We organize our collected generated summaries into three groups based on system type:

\begin{itemize*}
    \item \texttt{CNNDM Abs} denotes collected output summaries from abstractive systems.
    \item \texttt{CNNDM Ext} denotes collected output summaries from extractive systems.
    \item \texttt{CNNDM Mix} is the union of the two.
\end{itemize*}



\subsection{Representative Sample Selection}

% We obtain human judgements on system output summaries from 15 top-performing abstractive systems and 10 extractive systems on a representative sample of 100 documents from the \texttt{CNNDM} test set. 

% \pfliu{You can add some texts to describe why we should sample in this way~} \pg{Added some text, pls have a look.}
Since collecting human annotations is costly, we sample 100 documents out of the 11,490 documents in the \texttt{CNNDM} test set and evaluate system generated summaries of these 100 documents. We aim to include documents of varying difficulties in the representative sample. As a proxy to the difficulty of summarizing a document, we use the mean score received by the system generated summaries for the document. Based on this, we partition the \texttt{CNNDM} test set into $5$ equal sized bins.
Moreover, we aim to include documents whose summaries have a wide scoring range, as well as a narrow scoring range. To do this, we partition each of the $5$ bins further into $4$ equally sized bins based on the standard deviation of the metric scores received by the system summaries of a document. Finally, from each bin, we randomly sample one document. We repeat this process for 5 metrics (BERTScore, MoverScore, R-1, R-2, R-L) obtaining a sample of 100 documents. This methodology is further detailed in algorithm \ref{alg:sampling}. 

% we use two aspects to obtain a representative sample: the mean and standard deviations of the scores of each document's system summaries. A document's mean score represents the overall performance of systems on the document; and standard deviation represents the diversity in quality of system summaries generated for the document. Using document mean scores ensures that the sample contains a representative range of scores. Using standard deviation ensures that for the \textit{summary-level} setting, the sample contains documents with system summaries that span narrow and wide ranges of scores. 


% The sampling is done by dividing the test set documents into 5 bins based on their mean scores, and then further sub-dividing these bins into 4 sub-bins each according to standard deviation scores. A document is randomly sampled from each sub-bin. By repeating this 
% \gn{This algorithm can definitely go in the appendix if you need space.}

\begin{table*}[]%h!]
    \centering
    % \resizebox{\linewidth}{!}
    \small
    {
    \begin{tabular}{c}
        \toprule
        \begin{minipage}[t]{0.98\linewidth}
        \textbf{(a) Reference Summary}: 
        Bayern Munich beat Porto 6 - 1 in the Champions League on Tuesday. Pep Guardiola's side progressed 7 - 4 on aggregate to reach semi-finals. Thomas Muller scored 27th Champions League goal to pass Mario Gomez. Muller is now the leading German scorer in the competition. After game Muller led the celebrations with supporters using a megaphone. \\
        % Cesc Fabregas was caught by trailing arm of Stoke City Ace Charlie Adam . Former Barcelona Man picked up the injury during Chelsea's home win . Midfielder Adam scored wonder goal during the game but it wasn't enough . Fabregas took to Instagram to show he was all smiles despite the bruises . Click here for all the latest Chelsea News .\\
        \end{minipage}\tabularnewline
        % \midrule
        \begin{minipage}[t]{0.98\linewidth}
        \textbf{(b) System Summary (BART, \citet{lewis2019bart}):} 
        Bayern Munich beat Porto 6 - 1 at the Allianz Arena on Tuesday night. Thomas Muller scored his 27th Champions League goal. The 25 - year - old became the highest - scoring German since the tournament took its current shape in 1992. Bayern players remained on the pitch for some time as they celebrated with supporters. \\
        % Chelsea beat Stoke City 2 - 1 at Stamford Bridge on Saturday . Cesc Fabregas was caught in the face by Charlie Adam's flailing arm . The collision left the Spain international with a bloody nose . The 27 - year - old posted a picture to his Instagram account on Tuesday .\\
        \end{minipage}\tabularnewline 
        % \midrule
        \begin{minipage}[t]{0.98\linewidth}
        \textbf{(c) SCUs with corresponding evaluations}:  
        \vspace{-2\topsep}
        \begin{multicols}{2}
        \begin{itemize*}
            \item Bayern Munich beat Porto.~$\checkmark$
            \item Bayern Munich won  6 - 1.~$\checkmark$
            \item Bayern Munich won in Champions League.~$\checkmark$
            \item Bayern Munich won on Tuesday.~$\checkmark$
            \item Bayern Munich is managed by Pep Guardiola.~$\times$
            \item Bayern Munich progressed in the competition.~$\checkmark$
            \item Bayern Munich reached semi-finals.~$\times$
            \item Bayern Munich progressed 7 - 4 on aggregate.~$\times$
            \item Thomas Muller scored 27th Champions League goal.~$\checkmark$
            \item Thomas Muller passed Mario Gomez in goals.~$\times$
            \item Thomas Muller is now the leading German scorer in the competition.~$\checkmark$
            \item After the game Thomas Muller led the celebrations.~$\times$
            \item Thomas Muller led the celebrations using a megaphone.~$\times$
            % \item Cesc Fabregas plays for Chelsea.~$\times$ %\textit{(Not Present)}
            % \item Charlie Adam plays for Stoke City.~$\times$ %\textit{(Not Present)}
            % \item Cesc Fabregas used to play for Barcelona.~$\times$ %\textit{(Not Present)}
            % \item Charlie Adam injured Cesc Fabregas.~$\checkmark$ %\textit{(Present)}
            % \item Chelsea won against Stoke City.~$\checkmark$ %\textit{(Present)}
            % \item The match was at Chelsea's home.~$\times$ %\textit{(Not Present)}
            % \item Charlie Adam is a midfielder.~$\times$ %\textit{(Not Present)}
            % \item Charlie Adam scored a goal in the match.~$\times$ %\textit{(Not Present)}
            % \item Cesc Fabregas posted on instagram.~$\checkmark$ %\textit{(Present)}
            % \item Cesc Fabregas had bruises.~$\checkmark$ %\textit{(Present)}
            % \item Cesc Fabregas was smiling in the instagram post.~$\times$ %\textit{(Not Present)}
            % \item Charlie Adam's arm was trailing.~$\checkmark$ %\textit{(Present)}
    \end{itemize*}  
    \end{multicols}
    \end{minipage}\tabularnewline \\
                 % \midrule
    % \begin{minipage}[t]{0.98\linewidth}
    % \textbf{(d) Scores:} Human score: 53.85 (since 7/13 SCUs were ``present'') ; R-2: 8.62 ; R-1: 43.86; BScore: 41.51; MScore: 32.23.
    % \end{minipage}\tabularnewline 
    \bottomrule
    \end{tabular}
    }
    \caption{\label{tab:example_annotation}Example of a summary and corresponding annotation. (a) shows a reference summary from the represented sample of the \texttt{CNNDM} test set. (b) shows the corresponding system summary generated by BART, one of the abstractive systems used in the study. (c) shows the SCUs (Semantic Content Units) extracted from (a) and the ``\textit{Present}($\checkmark$)''/``\textit{Not Present}($\times$)'' marked by crowd workers when evaluating (b). 
    % (d) shows scores obtained in evaluating (b) against (a). It is interesting to note that due to the abstractive nature of the system summary, although it receives a high human score, it receives relatively low scores on the automatic metrics. 
    % Please see Sec.~\ref{sec:human_collection} for more details.
    }
\end{table*}



\subsection{Human Evaluation}

% \gn{I don't think you should use similarity to automatic evaluation metrics to motivate your choice of manual evaluation methods. It should be the other way around: you think of the underlying desiderata of ``good'' summaries for your application, create a human evaluation method that is able to capture these desiderata, then create an automatic evaluation method that serves as a good proxy for human evaluation. So please try to do the first two steps here.}

In text summarization, a ``good'' summary should represent as much relevant content from the input document as possible, within the acceptable length limits.
Many human evaluation methods have been proposed to capture this desideratum \cite{nenkova-passonneau-2004-pyramid-og,chaganty2018price,fan-etal-2018-controllable,litepyramids-shapira-etal-2019-crowdsourcing}.
Among these,  \emph{Pyramid} \cite{nenkova-passonneau-2004-pyramid-og,litepyramids-shapira-etal-2019-crowdsourcing} is a reliable and widely used method, that evaluates content selection by (1) exhaustively obtaining a set of Semantic Content Units (SCUs) from a set of reference summaries, (2) weighting them based on the number of times they are mentioned and (3) scoring a system summary based on which SCUs can be inferred from it. 
% However, although the Pyramid method can better capture a good summary's desiderata, it comes at the expensive cost of laborious manual work.

Recently, \citet{litepyramids-shapira-etal-2019-crowdsourcing} extend Pyramid to a lightweight, crowdsourcable method - LitePyramids, which uses Amazon Mechanical Turk~\footnote{https://www.mturk.com/} (AMT) for gathering human annotations. LitePyramids simplifies Pyramid by (1) allowing crowd workers to extract a subset of all possible SCUs and (2) eliminating the difficult task of merging duplicate SCUs from different reference summaries, instead using SCU sampling to simulate frequency based weighing. 

Both Pyramid and LitePyramid rely on the presence of multiple references per document to assign importance weights to SCUs. However in the \texttt{CNNDM} dataset there is only one reference summary per document. We therefore adapt the LitePyramid method for the single-reference setting as follows.
% We adopt this methodology and adapt it as detailed below for the one-reference-per-document setting, (in contrast to \citet{litepyramids-shapira-etal-2019-crowdsourcing}, who used it with multiple references per document in the DUC 2005 and 2006 datasets). It is worth nothing that a consequence of the single-reference-summary setting is that `importance'-based weighing of SCUs is no longer possible. 

% The human evaluation process involves three steps: SCU extraction, system evaluation and annotation scoring.

% and crowdsourceable version of the original Pyramid (a.k.a, LitePyramids technique), and demonstrated it on the DUC 2005 and 2006 multi-document summarization datasets.

% \gn{Also, you definitely need to explain the Pyramids technique and LitePyramids technique at least a little here, as some people may not know the details. Some of this explanation can be taken from the SCU extraction section and reference Table 2.}

% Since automatic evaluation metrics measure semantic equivalence between a system output text and a reference text, a content-selection-based approach such as Pyramid \cite{nenkova-passonneau-2004-pyramid-og} or LitePyramids~\cite{litepyramids-shapira-etal-2019-crowdsourcing} is suitable for obtaining human judgements.
% % for this purpose. 
% While the LitePyramids technique ~\cite{litepyramids-shapira-etal-2019-crowdsourcing} was designed for multiple reference summaries, the \texttt{CNNDM} dataset has only one reference summary per document. We adapt the LitePyramids technique to this setting by making some modifications. 


\paragraph{SCU Extraction} The LitePyramids annotation instructions define a Semantic Content Unit (SCU) as a \textit{sentence containing a single fact written as briefly and clearly as possible}.
Instead, we focus on shorter, more fine-grained SCUs that contain at most 2-3 entities. This allows for partial content overlap between a generated and reference summary, amd also makes the task easy for crowd workers. Please see Tab~\ref{tab:example_annotation} for an example. We exhaustively extract (up to 16) SCUs~\footnote{In our representative sample we found no document having more than 16 SCUs} from each reference summary.
Requiring the set of SCUs to be exhaustive increases the complexity of the SCU generation task, and hence instead of relying on crowd-workers, we create SCUs from reference summaries ourselves.
In the end, we obtained nearly 10.5 SCUs on average from each reference summary.

\paragraph{System Evaluation} During system evaluation the full set of SCUs is presented to crowd workers. Workers are paid similar to~\citet{litepyramids-shapira-etal-2019-crowdsourcing}, scaling the rates for fewer SCUs and shorter summary texts. For abstractive systems, we pay \$0.20 per summary and for extractive systems, we pay \$0.15 per summary since extractive summaries are more readable and might precisely overlap with SCUs. 
% Scaling down the rates used by \citet{litepyramids-shapira-etal-2019-crowdsourcing} to account for our relatively short SCU and summary texts and fewer SCUs, we paid workers \$0.20 per abstractive system summary evaluation task.
% We paid \$0.15 per extractive summary evaluation due to their higher readability and a higher chance of exact match with SCUs, in comparison with abstractive summaries.
We post-process system output summaries before presenting them to annotators by true-casing the text using Stanford CoreNLP \cite{manning-EtAl-2014-CoreNLP} and replacing ``unknown'' tokens with a special symbol ``$\Box$'' \citep{chaganty2018price}.

Tab.~\ref{tab:example_annotation} depicts an example reference summary, system summary, SCUs extracted from the reference summary, and annotations obtained on the SCUs in evaluating the system summary.

\paragraph{Annotation Scoring}
For robustness~\cite{litepyramids-shapira-etal-2019-crowdsourcing}, each system summary is evaluated by 4 crowd workers. Each worker annotates up to 16 SCUs by marking if an SCU is ``present" in a generated summary or ``not present". We obtain total 10,000 human annotations (100 documents~$\times$ 25 systems~$\times$ 4 workers). For each document, we identify a ``noisy" worker as one who disagrees with the majority (i.e. marks an SCU as ``present" when majority thinks ``not present" or vice-versa), on the largest number of SCUs. We remove the annotations of noisy workers and retain 7,742 annotations of the 10,000. After this filtering, we obtain an average inter-annotator agreement (Krippendorff's alpha~\cite{krippendorff2011computing}) of 0.66.
% \pg{suggestion: remove word 'overall'}
\footnote{The agreement was 0.57 and 0.72 for extractive and abstractive systems respectively.}
Finally, we use the majority vote to mark the presence of an SCU in a system summary, breaking ties by the class, ``not present".
% \pg{suggestion: s/majority class/class}



% Please refer to Tab~\ref{tab:anno_details}. for more details.
% \begin{table}[h]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{|c|c|}
%         \toprule
%         Number of documents & 100 \\
%         Number of systems & 25 \\
%         Avg. SCUs per document & -\\
%         Number of annotations & 10000 \\
%         Number of filtered annotations & - \\
%         Avg errors in `noisy' annotations & -\\
%         Avg errors in filtered annotations & -\\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{\label{tab:anno_details} Properties of the collected dataset}
% \end{table}



% following the LitePyramids recommendation.


% Our primary purpose in obtaining human evaluations on state-of-the-art summarization system outputs is to create a meta-dataset to evaluate the performance of automatic metrics like ROUGE and BertScore. By design, such metrics measure the semantic equivalency between a system output text and a reference text. Thus, a content-selection-based approach is suitable for obtaining human judgements for this purpose. 

% We achieve this by using the LitePyramids approach with some modifications. \citet{litepyramids-shapira-etal-2019-crowdsourcing} demonstrate LitePyramids on the DUC 2005 and 2006 multi-document summarization datasets, where each document has 4 reference summaries, each being 250 words in length on average. Moreover, the system outputs in the DUC datasets are extractive.\pg{need to confirm this.} We adapt the LitePyramids approach to our setting, in which abstractive systems have performed single-document summarization on the \texttt{CNN/DailyMail} dataset. In this dataset, each document has a single reference per document, which is on average 56 tokens in length. With this in mind, we make the following changes to adapt LitePyramids:

% With this in mind, we make the following changes to adapt LitePyramids:
% \begin{itemize}
%     \item We reinstate the need to exhaustively extract SCUs, to mine as much content as possible from the single reference summary. We aim to obtain up to 16 SCUs from each reference summary.
%     \item We also focus on extracting shorter and more fine-grained SCUs, trying to limit each SCU (to the extent possible) to 2-3 concepts, such as the relationship between two entities. We find that the longer SCUs in the LitePyramids dataset are too coarse-grained to be inferred from most abstractive system summaries.
%     \item During system evaluation, we evaluate each system summary against the full set of (up to 16) SCUs extracted from the correspponding reference summary. Unlike LitePyramids, sampling is not performed, due to the relative scarcity of SCUs.  
% \end{itemize}.

% Due to these changes, the first task (Pyramid creation) requires skilled work. This was performed by graduate students in our department. \pg{We aim to perform this across 100 documents. So far, we have performed this for 21 documents, obtaining an average of 13 SCUs per document} 

% The second task is \pg{going to be} performed by crowdworkers on AMT. Using the LitePyramids methodology, we evaluate each output summary with its full set of SCUs, and we assign each such evaluation to five workers. Using voting between the 5 workers on each SCU improves the robustness of the evaluation.

% \subsection{Human Evaluation: Results}
% We show \pg{once we have the results}:
% \begin{itemize}
%     \item Agreement between the recall variant of each automated metric and human evaluation scores on both summary-level and system-level evaluation. \mb{We should focus primarily on the F variant because that's what we use throughout. We can add recall variant in the appendix.}
%     \item Variation in this agreement w.r.t various properties, similar to those reported earlier, now with human evaluations in the mix.
% \end{itemize}








==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}
% \pfliu{Just wrote a draft for intro. Please feel free to modify anything!!}
% \gn{Maybe first discuss that manual evaluation (such as the pyramid method) is the gold standard first before going into this next sentence?}

\begin{table*}[h]
    \centering
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
        \toprule
        Experiment & Research Question & Observation  \\
        \midrule
        I (Sec. \ref{sec:williams_test})
        & 
        \begin{minipage}[t]{\columnwidth}
        Can metrics reliably rank summarization systems?
        Which metrics are better correlated with human judgements at this task, with statistical significance?
        \end{minipage}
        &
        \begin{minipage}[t]{\columnwidth}
        None of the metrics significantly outperform others across all datasets. For abstractive systems on \texttt{CNNDM}, ROUGE based metrics are significantly better than others.
        \end{minipage} \\
        \midrule
        II (Sec. \ref{sec:topk_human})
        & 
        \begin{minipage}[t]{\columnwidth}
        Can metrics reliably quantify the improvements made by high quality systems over other competitive systems? 
        % (System-level Pearson's correlation on top-k systems) 
        \end{minipage}
        & 
        \begin{minipage}[t]{\columnwidth}
        No, especially for abstractive and extractive systems on \texttt{CNNDM}.
        \end{minipage} \\
        \midrule
        % III (Sec. \ref{sec:quality_human})
        % & 
        % \begin{minipage}[t]{\columnwidth}
        % Can metrics reliably quantify the improvements made by low, medium and high quality systems?
        % \end{minipage}
        % &
        % \begin{minipage}[t]{\columnwidth}
        % Metrics are more reliable when quantifying improvements on low quality systems as compared to medium or high quality systems.
        % \end{minipage} \\
        % \midrule
        V (Sec. \ref{sec:bootstrap})
        &
        \begin{minipage}[t]{\columnwidth}
        Can metrics reliably say if one system is significantly better than another?
        \end{minipage}
        &
        \begin{minipage}[t]{\columnwidth}
        Overall, yes. On the CNNDM dataset, R-2 is most reliable to compare abstractive systems and R-1 to compare extractive systems; and on the TAC dataset, MoverScore can be used to compare systems.
        \end{minipage} \\
        \midrule
        I (Sec. \ref{sec:summ_level_human}) & 
        \begin{minipage}[t]{\columnwidth}
        How do metrics correlate with human judgements in ranking top scoring summaries?
        \end{minipage}
        & 
        \begin{minipage}[t]{\columnwidth}
        Metrics have lower correlation with human judgments at the summary level as compared to system level.
        \end{minipage}  \\
        \bottomrule
    \end{tabular}
    }
    \caption{\label{tab:expt_summary} Summary of our experiments and observations. Please see section~\ref{sec:experiments} for more details. \mb{Needs to be updated after final results.}}
\end{table*}




In text summarization, \emph{manual evaluation}, as exemplified by the Pyramid method \cite{nenkova-passonneau-2004-pyramid-og}, is the gold-standard in evaluation.
However, due to time required and relatively high cost of annotation, 
%In text summarization, 
the great majority of research papers on summarization use exclusively automatic evaluation metrics, such as ROUGE \cite{lin2004rouge}
% \gn{I think it's worth mentioning that ROUGE is \emph{by far} the most popular of these metrics, and people often use it without thinking about it too carefully}
, JS-2~\cite{js2}, S3~\cite{peyrard_s3}, BERTScore~\cite{bert-score}, MoverScore~\cite{zhao-etal-2019-moverscore} etc.
Among these metrics, ROUGE is by far the most popular, and there is relatively little discussion of how ROUGE may deviate from human judgment and the potential for this deviation to change conclusions drawn regarding relative merit of baseline and proposed methods.
To characterize the relative goodness of evaluation metrics, it is necessary to perform \emph{meta-evaluation} \cite{graham-2015-evaluating,lin-och-2004-orange}, where a dataset annotated with human judgments (e.g.~TAC~\footnote{https://tac.nist.gov/} 2008~\cite{tac2008}) is used to test the degree to which automatic metrics correlate therewith.
% (Figure XX. illustrate the general workflow.) \mb{what kind of figure do we want to put here?}

% However, this classic meta-evaluation dataset from TAC is arriving at a plateau \gn{``arriving at a plateau'' is not clear. Do you mean something like ``the classic TAC meta-evaluation dataset is now XXX years old, and it is not clear whether conclusions found there will hold with modern systems and summarization tasks''}

However, the classic TAC meta-evaluation datasets are now 6-12 years old~\footnote{In TAC, summarization was in 2008, 2009, 2010, 2011, 2014. In 2014, the task was biomedical summarization.}
% \pfliu{should we add a footnote like: ``In TAC, summarization was in 2008, 2009, 2010, 2011, 2014. In 2014, the task was biomedical summarization.''}, 
% \pfliu{We should check the newest TAC} \mb{In TAC, summarization was in 2008, 2009, 2010, 2011, 2014. In 2014, the task was biomedical summarization. I think saying nearly 10 years is fine here.}, 
and it is not clear whether conclusions found there will hold with modern systems and summarization tasks.
% due to the rapid development both in summarization systems and datasets.
Two earlier works exemplify this disconnect:
(1) \citet{peyrard-2019-studying} observed that the human-annotated summaries in the TAC dataset are mostly of lower quality than those produced by modern systems and that various automated evaluation metrics strongly disagree in the higher-scoring range in which current systems now operate.
(2) \citet{rankel-etal-2013-decade} observed that the correlation between ROUGE and human judgments in the TAC dataset decreases when looking at the best systems only,
even for systems from eight years ago, which are far from today's state-of-the-art.
% \gn{``even for systems from XXX years ago, which are far from today's state-of-the-art''}.

Constrained by few existing human judgment datasets, it remains unknown how existing metrics behave on current state-of-the-art summarization systems.
In this paper, we ask the question: ``does the rapid progress of model development in summarization models require us to \emph{re-evaluate} our evaluation process for text summarization?''

% \gn{I would describe the experimental setup first, which is impressive because you've created evaluations for so many systems.} \pfliu{Great suggestion!}
To this end, we create and release a large benchmark for meta-evaluation of summarization metrics including:%
% \mb{Can we enumerate this? Makes it easier for reviewers to count our contributions} \gn{Yes, I think this is good. If you want to save space you can reduce the indentation and spacing between the bullets.}

\begin{itemize*}
    % \item \textbf{Outputs} from 25 state-of-the-art extractive (e.g.~matchSum~\cite{zhong2020extractive}) and abstractive (e.g.~T5~\cite{raffel2019exploring-t5}, ~BARTSum~\cite{lewis2019bart}) summarization systems on the \texttt{CNN/DailyMail}.
    % \gn{The "e.g.s" here did not provide a lot of value, and were kind-of verbose. I removed them.}
    \item \textbf{Outputs} from 25 top-scoring extractive and abstractive summarization systems on the \texttt{CNN/DailyMail} dataset.
    %\mb{We have 25 outputs from sota systems on cnn/dm and 10 on xsum.}
    \item \textbf{Automatic evaluations} from a number of existing evaluation metrics including more traditional metrics (e.g.~ROUGE~\cite{lin2004rouge}) and modern semantic matching metrics (e.g.~BertScore~\cite{bert-score}, MoverScore~\cite{zhao-etal-2019-moverscore}. 
    % FactCC~\cite{kryciski2019factcc-socher}).
    \item \textbf{Manual evaluations} using the lightweight pyramids method~\cite{litepyramids-shapira-etal-2019-crowdsourcing}, which we use as a gold-standard for evaluating these summarization systems as well as automated metrics.
\end{itemize*}


% \begin{description}
%     \item[Outputs] from 15 state-of-the-art extractive (e.g.~matchSum~\cite{zhong2020extractive}) and abstractive (e.g.~T5~\cite{raffel2019exploring-t5}, ~BARTSum~\cite{lewis2019bart}) summarization systems on the \texttt{CNN/DailyMail} and \texttt{XSum} datasets,
%     \item[Automatic evaluations] from a number of existing evaluation metrics including more traditional metrics (e.g.~ROUGE~\cite{lin2004rouge}), modern semantic matching metrics (e.g.~BertScore~\cite{bert-score}, MoverScore~\cite{zhao-etal-2019-moverscore}, FactCC~\cite{kryciski2019factcc-socher}).
%     %, which attempts to check for factual consistencies, and \gn{cite all of these}
%     \item[Manual evaluations] using the lightweight pyramids method~\cite{litepyramids-shapira-etal-2019-crowdsourcing}, which we can use as a gold-standard for evaluating these summarization systems.
% \end{description}


% \gn{For all of the research questions below, it might be nice to make a contrast with what was known before on the TAC dataset. For example, on the TAC dataset maybe ROUGE's correlations with human evaluation were OK, and the other metrics were better? Maybe re-write a little bit} \pfliu{have made the first-pass modification of the following questions.}
Using this benchmark, we perform an extensive analysis, which indicates the need to re-examine our assumptions about evaluation of automatic summarization systems.
Specifically we conduct four experiments to investigate which metrics are reliable. Detailed experimental settings and our main observations are summarized in Tab.~\ref{tab:expt_summary}.



% \pfliu{As Graham suggested, we can focus on Q3. And Graham's de-correlation idea is super-cool, we can put it in our future work section?} \mb{I agree, it's a very interesting idea}
% \gn{Honestly, I don't really care all that much about whether metrics correlate with each-other. The really important thing is whether they correlate with human judgement, as that will allow us to choose which metrics we should be using to assess our methods in the future. Maybe we can focus on the results regarding correlation with human judgement be the main ones we emphasize (in other words, mainly talk about RQ3). I think we could mention the de-correlation of the evaluation metrics as a side-note. \emph{However}, not necessarily for this current submission deadline, but maybe to think about for later: it would be particularly interesting if we could use de-correlation of metrics to indicate whether they will indeed disagree with human evaluation. In other words if we could demonstrate ``in situations where metrics correlate well with each-other we can expect that these correlated metrics will also likely match with human eval''. That way we could occasionally check to make sure that our allegedly best metrics continue to be correlated on top systems, and if they start de-correlating we'll know we have to run a meta-eval to determine which metrics are still OK to use.}

% \paragraph{RQ1:}  How do automated metrics correlate when ranking different summaries of different scoring ranges? And which factors matter for their correlation?
% We revisit the experiments of~\citet{peyrard-2019-studying} that concludes automated metrics strongly disagree for ranking high-scoring summaries.
% %and perform a more fine-grained analysis of the factors affecting correlation of metrics. 
% We generalize this setting to more datasets, and find that not only do metrics disagree in the top scoring range, they often also disagree in the low and average scoring range. 



% By generalizing this setting to more datasets, to our surprise, we find that not only do metrics disagree in the top scoring range, they often also disagree in the low and average scoring range. 
% \pfliu{Feel free to check if above statements are appropriate. Especially, two points: 1) should we highlight some observations with respect to `` And which factors matter for their correlation''? 2) is this a clear statement: ``By generalizing this setting to more datasets,''. } 
% \mb{I think both are fine. But, it seems that in the top scoring range (sota abs, ext) correlations are high.}
% \pfliu{We can revise above statement once we finish all experiments.}
% correlated behavior among automatic metrics in the appropriate scoring range that evaluation metrics that behave similarly on these datasets (average-scoring range) strongly disagree in the higher-scoring range in which current systems now operate.

% By more carefully experimental design, we find some limitation of current experiment settings:

% 1) XXX (e.g., simulate the higher-scoring range in an improper way)
% 2) XXX
% 3) XXX
% ...

% \paragraph{RQ2:} How do different metrics correlate when ranking different top systems?
% \mb{Since we've already motivated the need for our work above, maybe the next part can be removed?}
% The proliferation of neural network-based summarization systems frequently updates the state-of-the-art results on benchmark datasets.
% This makes it more essential
% % \mb{Maybe we can say ``essential" instead of more attractive?}
% to re-examine and generalize the observation obtained eight years ago \cite{{rankel-etal-2013-decade}} that correlation between ROUGE and human judgments in the TAC dataset decreases on top-ranked systems.


% It would be useful to reveal the correlation behavior between different metrics on top-k systems for various values of k.

% observed that the correlation betweenROUGE and human judgments in the TAC datasetdecreases

% \paragraph{RQ3:} Which metrics are more reliable?
% \mb{Again, I think the motivation for this has been provided above and the next part can be removed. Maybe we can add our general observation here as done for RQ1?}
% One major limitation of the existing human judgment dataset is that it is created based on systems at that time, (e.g., TAC 2008), on which we conclude that ROUGE correlate above-moderate with human judgment while MoverScore performs best.
% The absence of human judgments on current advanced systems and abstractive models hinders our complete understanding of existing automatic metrics.


% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{ccllr}
% \cmidrule{1-4}    \multicolumn{1}{l}{\textbf{M-Evaluation}} & \multicolumn{1}{l}{\textbf{Question}} & \textbf{Setting} & \textbf{Experiment} &  \\
% \cmidrule{1-4}    \multicolumn{1}{l}{\multirow{2}[2]{*}{HJ-free}} & Q1    & Summary-level & scoring range &  \\
%           & Q2    & System-level & scoring range &  \\
% \cmidrule{1-4}    \multirow{5}[2]{*}{HJ-aware} & \multirow{5}[2]{*}{Q3} & Summary-level & correlation &  \\
%           &       & \multirow{4}[1]{*}{Summary-level} & topk systems &  \\
%           &       &       & scoring range &  \\
%           &       &       & William test &  \\
%           &       &       & Pairwise model ranking &  \\
% \cmidrule{1-4}    \end{tabular}%
%   \label{tab:addlabel}%
% \end{table*}%



% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \footnotesize
%     \begin{tabular}{lcll}
%     \toprule
%     \textbf{M-Eval} & \multicolumn{1}{l}{\textbf{Question}} & \multicolumn{1}{l}{\textbf{Setting}} & \textbf{Experiment} \\
%     \midrule
%     \multirow{2}[2]{*}{\emph{HJ-free}} & Q1    & \multicolumn{1}{l}{Summary-level} & scoring range \\
%           & Q2    & \multicolumn{1}{l}{System-level} & scoring range \\
%     \midrule
%     \multirow{5}[4]{*}{\emph{HJ-aware}} & \multirow{5}[4]{*}{Q3} & \multicolumn{1}{l}{Summary-level} & correlation \\
% \cmidrule{3-4}          &       & \multirow{4}[2]{*}{System-level} & top-$k$ systems \\
%           &       &       & scoring range \\
%           &       &       & William test \\
%           &       &       & model ranking \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
%     \caption{Outline of our experiment designs. \textbf{M-Eval} represents Meta-evaluation and ``\textit{HJ}'' denotes human judgement. \pfliu{It's still a prototypical outline, feel free to edit. Finally, we should also add section number to it.}}
% \end{table}%







% \pfliu{Following statements can be compressed and more detailed could be put in Meta Evaluation Setting.} \mb{Hi Pengfei, is the following fine? Please feel free to make any changes}

% Our contributions can be summarized as follows:
% \begin{enumerate}
%     \item We conduct a fine-grained analysis of summarization evaluation metrics both at a summary-level as well as system-level.
%     \item We analyze summaries generated by state-of-the-art extractive and abstractive systems\footnote{All system output was obtained from the original authors} on modern datasets \texttt{CNN/DailyMail} and \texttt{XSum} \pg{all results on cnn-dm so far, x-sum is work in progress}.
%     \item We extend the meta-evaluation setup to include modern semantic matching metrics like BertScore, and MoverScore as well as FactCC, which checks for factual consistencies.
%     \item We conduct a manual summary evaluation (pyramid method) of the top 15 advanced systems on the CNN/DailyMail dataset, and make these collected human judgments publicly available.
% \end{enumerate}



% To generalize the conclusions drawn by \citet{peyrard-2019-studying}, we augment their experiments in multiple ways:
% \begin{itemize}
%     \item Datasets: besides \texttt{TAC-2008}, \texttt{TAC-2009}, we additionally use \texttt{CNN/DailyMail} \cite{nallapati-etal-2016-abstractive} and \texttt{XSum} \cite{narayan2018don} which are popular datasets to train and evaluate modern summarization models.
%     \item Systems: We pick typical neural summarization systems, including the state-of-the-art models. Additionally, we also use the genetic algorithm~\cite{peyrard-eckle-kohler-2016-general} used by \citet{peyrard-2019-studying} to simulate future research in extractive summarization and generate extractive summaries from the full scoring range.
%     \item Metrics: In terms of evaluation metrics, we additionally use ROUGE 1, BERTScore\cite{bert-score}, MoverScore\cite{zhao-etal-2019-moverscore}, and the FactCC factuality metric \cite{kryciski2019factcc-socher}.  \mb{FactCC evaluation is in progress}.
%     \item Evaluation Setting: In addition to summary-level evaluation, we also consider the system-level evaluation setting.
% \end{itemize}
% ...


% \subsection{Characteristics of Our Work}
% \begin{itemize}
%     \item Observe some inconsistent results with  Peyrard's work.
%     \item We present a more generalized conclusion based on a comprehensive experimental settings.
%     \item Beyond the summary-level evaluation, we conduct fine-grained analysis under system-level setting.
%     \item We conduct a manual summary evaluation (pyramid method) of 15 systems on CNNDM, and make these collected human judgments publicly available.
% \end{itemize}



==> meta-eval.tex <==
% \subsection{Meta Evaluation Settings}
\subsection{Evaluation Metrics}
\label{sec:metrics}
%\pfliu{Probably, one or two more metrics?}
We examine eight metrics that measure the agreement between two texts, in our case, between the system summary and reference summary: 
% \pg{todo: link the metrics for the repos, to fulfill reproducability checklist}

\pfliu{Try composite metrics: ``average(R1, R2, RL)'', ``average(all)''}

\noindent\textbf{BERTScore (BScore)} measures soft overlap between contextual BERT embeddings of tokens between the two texts\footnote{Used code at \href{https://github.com/Tiiiger/bert_score}{github.com/Tiiiger/bert\_score}} \citep{bert-score}.

\noindent\textbf{MoverScore (MScore)} applies a distance measure to contextualized BERT and ELMo word embeddings\footnote{Used code at \href{https://github.com/AIPHES/emnlp19-moverscore}{github.com/AIPHES/emnlp19-moverscore}} \citep{zhao-etal-2019-moverscore}.

\noindent\textbf{Word Mover Similarity (WMS)} measures similarity using minimum distance matching between texts which are represented as a bag of word embeddings\footnote{WMS and SMS are calculated using the code provided at \href{https://github.com/eaclark07/sms}{github.com/eaclark07/sms}} \citep{kusner2015word}.

% \item \textbf{S3}: We have not used this
\noindent\textbf{Sentence Mover Similarity (SMS)} applies minimum distance matching between text \citep{clark2019sentence} based on sentence embeddings.
%represented as a bag of sentence embeddings .

\noindent\textbf{ROUGE-1 and ROUGE-2}\ measure overlap of unigrams and bigrams respectively\footnote{\label{pyrouge}For ROUGE-1,2, and L evaluation, we used the pyrouge wrapper: \href{https://github.com/bheinzerling/pyrouge}{github.com/bheinzerling/pyrouge}} \citep{lin2004rouge}.

\noindent\textbf{ROUGE-L} measures overlap of the longest common subsequence between two texts \citep{lin2004rouge}.

\noindent\textbf{JS divergence (JS-2)} measures Jensen-Shannon divergence between the two text's bigram distributions\footnote{JS divergence is calculated using the function defined in \href{https://github.com/UKPLab/coling2016-genetic-swarm-MDS}{github.com/UKPLab/coling2016-genetic-swarm-MDS}} \citep{lin-etal-2006-information}. 


% \aash{check if new metrics are correct}


\noindent
We use the recall variant of all metrics (since the Pyramid method of human evaluations is inherently recall based) except MScore which has no specific recall variant.


% We went with recall since the pyramid method of human evaluations is inherently recall based (find number of SCUs in rhe reference that are implied by the generated summary)
%\gn{Mention because this is because the pyramid method is also recall-based}.

% \paragraph{FactCC} \cite{kryciski2019factcc-socher} is a weakly-supervised BERT-based measure of factual consistency at a document-sentence level. \mb{Maybe it shouldn't be here?}

\subsection{Correlation Measures}

%\subsubsection{Direct}

\noindent\textbf{Kendall's tau} is a measure of correspondence between two rankings \citep{kendall-tau}. It accepts two lists of rankings as input and takes a value between -1 and 1 to reflect the level of agreement between the two rankings.
%We used its definition as given in \citet{kendall-tau-2} and as implemented by \citet{scipy-2020}. \mb{Can be removed to save space since all of our results use Pearson's correlation.}

\noindent\textbf{Pearson's Correlation}
%\mb{I can't find the right citation}
is a measure of linear correlation between two variables and is popular in meta-evaluating metrics at the system level \citep{lee1988thirteen}. We use the implementation given by~\citet{scipy-2020}.

\noindent\textbf{Williams' Significance Test} is a means of calculating the statistical significance of differences in correlations for dependent variables \cite{williams-test,graham-baldwin-2014-testing}. This is useful for us since metrics evaluated on the same dataset are not independent of each other.


\subsection{Meta Evaluation Strategies}
\label{sec:meta_eval_strategy}
There are two broad meta-evaluation strategies - summary level and system level.

\paragraph{Setup:} For each document $d_i, i \in \{1 \dots n\}$ in a dataset $\mathcal{D}$, we have $J$ system outputs, where the outputs can come from (1) extractive systems (Ext), (2) abstractive systems (Abs) or (3) a union of both (Mix). Let $s_{ij}, j \in \{1 \dots J\}$ be the $j^{th}$ summary of the $i^{th}$ document.

\subsubsection{Summary level}
Correlation at the summary level is calculated as follows:
\begin{equation}
    \begin{split}
        K_{m_1 m_2}^{sum} &= \frac{1}{n} \sum_{i = 1}^{n} \bigg( K\big([m_1(s_{ij}) \dots m_1(s_{iJ})], \\
        & ~~~~~~~~~~~~~~~~~~~~~~~~[m_2(s_{ij}) \dots m_2(s_{iJ}) ]\big) \bigg)
    \end{split}
    \label{eqn:summ_level_corr}
\end{equation}
where $m_i$ represent a specific metric. Here, correlation is calculated for each document, among the different system outputs of that document, and the mean value is reported.
% \begin{align}
%         K_{m_1 m_2}^{sum} &= \frac{1}{n} \sum_{i = 1}^{n} \bigg[ K([m_1(s_{ij}): j \in \{1 \dots m \}], [m_2(s_{ij}): j \in \{1 \dots m \}]) \bigg]
% \end{align}



% \pfliu{Definition of $m_1$()}
% \paragraph{Cross-sample}
% \paragraph{Within-sample}

\subsubsection{System level}
Correlation at the system level is calculated as follows:
\begin{equation}
\resizebox{0.95\hsize}{!}{%
        \begin{split}
        K_{m_1 m_2}^{sys} &= K\bigg( \left[\frac{1}{n}\sum_{i = 1}^n m_1(s_{ij}) \dots \frac{1}{n}\sum_{i = 1}^n m_1(s_{iJ})\right], \\
        & ~~~~~~~~~~~~\left[\frac{1}{n}\sum_{i = 1}^n m_2(s_{ij}) \dots \frac{1}{n}\sum_{i = 1}^n m_2(s_{iJ})\right]\bigg)
    \end{split}
    }
\end{equation}
where $m_i$ represents a specific metric. Additionally, the ``quality" of a system $Sys_j$ is defined as the mean human score received by it i.e. 
\begin{equation}
    \mathrm{HScore}_{mean}^{sys_j} = \frac{1}{n}\sum_{i=1}^{n} \mathrm{humanScore}(s_{ij})
    \label{eqn:human_score}
\end{equation}
% Here, correlation is calculated betweeen different systems which are ranked based on the mean score received by a system.

==> related_work.tex <==
\section{Related Work}

% \gn{Move this after the experiments. Don't want to break the flow of the paper.}
This work is connected to the following threads of topics in text summarization.

% \pfliu{Related Work Section could be more condensed}
% \pfliu{It seems more summary-level works should be included, I put some here: 
% 1) The price of debiasing automatic metrics in natural language evaluation
% 2) Better Rewards Yield Better Summaries: Learning to Summarise Without References
% 3) Learning to Score System Summaries for Better Content Selection Evaluation [This paper gives a good formulate of summary-level definition, we can refer to it.]
% }

\paragraph{Human Judgment}
Despite many approaches to the acquisition of human judgment \cite{chaganty2018price,nenkova-passonneau-2004-pyramid-og,litepyramids-shapira-etal-2019-crowdsourcing,fan-etal-2018-controllable}, \textit{Pyramid} \cite{nenkova-passonneau-2004-pyramid-og} has been a mainstream method to meta-evaluate various automatic metrics.
Specifically, Pyramid provides a robust technique for evaluating content selection by exhaustively obtaining a set of Semantic Content Units (SCUs) from a set of reference summaries, and then scoring system summaries on how many SCUs can be inferred from them. Recently, \citet{litepyramids-shapira-etal-2019-crowdsourcing} proposed a lightweight and crowdsourceable version of the original Pyramid (a.k.a, LitePyramids technique), and demonstrated it on the DUC 2005 and 2006 multi-document summarization datasets.
In this paper, our human evaluation methodology is based on the Pyramid \cite{nenkova-passonneau-2004-pyramid-og} and LitePyramids \cite{litepyramids-shapira-etal-2019-crowdsourcing} techniques.
%SCUs are weighted based on how many reference summaries they appear in. This provides for a robust measure of content selection, but is rarely used due to the need for skilled human evaluation.


 
% Recently,
% LitePyramids achieves this by (i) removing the constraint that SCU extraction is exhaustive; (ii) eliminating the difficult task of merging duplicate SCUs from different reference summaries; and (iii) sampling from the set of SCUs instead of explicitly assigning importance weights. They divide the process into two AMT tasks: (i) Pyramid creation, in which SCUs are obtained from reference summaries, and (ii) System summary evaluation using the created SCUs. The final score of a system summary is the percentage of SCUs that it matched.




\paragraph{Meta-evaluation with Human Judgment}
The effectiveness of different automatic metrics - ROUGE-2~\cite{lin2004rouge}, ROUGE-L~\cite{lin2004rouge}, ROUGE-WE~\cite{ng-abrecht-2015-better}, JS-2~\cite{js2} and S3~\cite{peyrard_s3}
is commonly evaluated based on their correlation with human judgments (e.g., on the TAC 2008~\cite{tac2008} and TAC 2009~\cite{tac2009} datasets).
%on the TAC 2008~\cite{tac2008} and TAC 2009~\cite{tac2009} .
As an important supplementary technique to meta-evaluation, \citet{graham-2015-evaluating} advocate for the use of a significance test, William's test~\cite{williams-test}, to measure the improved correlations of a metric with human scores and show that the popular variant of ROUGE (mean ROUGE-2 score) is sub-optimal. 

Unlike these works, instead of proposing a new metric, in this paper, we upgrade the meta-evaluation environment by introducing a sizeable human judgment dataset evaluating current state-of-the-art systems and mainstream datasets. And then, we re-evaluate diverse metrics at both system and summary level settings.

% Recently, \citet{ma-etal-2019-results} showed that as the set of summarization systems grows stronger, the correlation between machine translation evaluation metrics decreases. In this paper, we analyze whether this behaviour is also exhibited by summarization evaluation metrics for the current best systems.


% Typically, existing works perform meta-evaluation mainly from two types of settings: \textit{system-level} and \textit{summary-level}.

% Most metrics have been shown to be highly correlated with human judgments at the system level on the TAC 2008, TAC 2009 datasets. However, evaluation metrics show poor correlations with human judgments on the top systems~\cite{rankel-etal-2013-decade}. \citet{graham-2015-evaluating} show that the popular variant of ROUGE (mean ROUGE-2 score) is sub-optimal and advocate for the use of a significance test, William's test~\cite{williams-test}, to measure the improved correlations of a metric with human scores.

% Recently, \citet{ma-etal-2019-results} showed that as the set of summarization systems grows stronger, the correlation between machine translation evaluation metrics decreases. In this paper, we analyze whether this behaviour is also exhibited by summarization evaluation metrics for the current best systems.





\paragraph{Meta-evaluation without Human judgment}
% The expensive annotation cost of human judgment-based meta-evaluation encourages researchers to explore evaluation methods that don't rely on human judgments. 
% For example, 
% instead of directly accessing which metrics are reliable,
\citet{peyrard-2019-studying} meta-evaluates metrics without human judgments by analyzing the correlations between different automatic summarization evaluation metrics
on the TAC 2008 and TAC 2009 datasets using system summaries synthetically generated by an extractive Genetic Algorithm~\cite{peyrard_genetic}, which simulates the whole scoring range. In this setting, they observe that metrics disagree with each other in the high scoring range.

% In this paper, even when we have already created new human judgments, we still re-evaluate existing metrics under the human judgment-free setting due to:
% 1) we observe some results that are not entirely consistent with \citet{peyrard-2019-studying}'s observations.
% 2) we revise \citet{peyrard-2019-studying}'s conclusion by a more generalized setting.
% \pfliu{Above two points probably should be modified.}


% Meta evaluation of summarization metrics is typically performed either on the \textit{summary level} or \textit{system level}

% \cite{s3-peyrard-etal-2017-learning}.

% \cite{s3-peyrard-etal-2017-learning} define two settings in which meta-evaluation of evaluation metrics can be done: \textit{system-level correlation} and \textit{summary-level correlation}, which we revisit in \ref{sec:meta_eval_strategy}.  They propose a new learned evaluation metric which combines existing metrics to maximize  summary-level correlation with human judgments.

% \paragraph{Summary level meta-evaluation} was recently performed by \citet{peyrard-2019-studying}. They analyze the correlations between five automatic summarization evaluation metrics
% - ROUGE-2~\cite{lin2004rouge}, ROUGE-L~\cite{lin2004rouge}, ROUGE-WE~\cite{ng-abrecht-2015-better}, JS-2~\cite{js2} and S3~\cite{peyrard_s3}
% on the TAC 2008~\cite{tac2008} and TAC 2009~\cite{tac2009} datasets using system summaries synthetically generated by an extractive Genetic Algorithm~\cite{peyrard_genetic} which simulates the whole scoring range. In this setting, they observe that metrics disagree with each other in the high scoring range.

% \citet{bohm2019better} measure correlation at a summary level on the CNN/Daily Mail dataset between automatic metrics and human judgment scores collected by \citet{chaganty2018price}. They find that automatic metrics were poor predictors of which summaries humans would consider ``good".

% \paragraph{System level meta-evaluation}
% % \pfliu{The first sentence is a little confused.}
% % Even though automatic evaluation metrics inherently measure the quality of a generated summary, they are also used to evaluate summarization systems, typically by measuring the mean score received by a system.
% Most metrics have been shown to be highly correlated with human judgments at the system level on the TAC 2008, TAC 2009 datasets. However, evaluation metrics show poor correlations with human judgments on the top systems~\cite{rankel-etal-2013-decade}. \citet{graham-2015-evaluating} show that the popular variant of ROUGE (mean ROUGE-2 score) is sub-optimal and advocate for the use of a significance test, William's test~\cite{williams-test}, to measure the improved correlations of a metric with human scores.

% Recently, \citet{ma-etal-2019-results} showed that as the set of summarization systems grows stronger, the correlation between machine translation evaluation metrics decreases. In this paper, we analyze whether this behaviour is also exhibited by summarization evaluation metrics for the current best systems.

% \paragraph{Human evaluations} 

% \citet{chaganty2018price} also obtain human evaluations on system summaries on the CNN/Daily Mail dataset, but with a focus on language quality of summaries. They collect human judgments on \emph{fluency}, \emph{redundancy} and \emph{overall quality} on 3-point Likert scales. In comparison, our work is focused on evaluating content selection, which is more closely aligned with the task of text similarity measurement that automatic metrics aim to perform. Their evaluation covers 4 abstractive systems, with the aim of combining human and automatic metrics to obtain a low-cost unbiased estimator. In contrast, ours work focuses on comprehensively comparing the reliability of automatic metrics by collecting human judgments across 15 abstractive systems. 

% Our human evaluation methodology is based on the Pyramid \cite{nenkova-passonneau-2004-pyramid-og} and LitePyramids \cite{litepyramids-shapira-etal-2019-crowdsourcing} techniques. Pyramid provides a robust technique for evaluating content selection by exhaustively obtaining a set of Semantic Content Units (SCUs) from a set of reference summaries, and then scoring system summaries on how many SCUs can be inferred from them. SCUs are weighted based on how many reference summaries they appear in. This provides for a robust measure of content selection, but is rarely used due to the need for skilled human evaluation.

% The LitePyramids technique \cite{litepyramids-shapira-etal-2019-crowdsourcing}, proposed a lightweight, sampling-based, and crowdsourceable version of the original Pyramid, and demonstrated it on the DUC 2005 and 2006 multi-document summarization datasets. LitePyramids achieves this by: (i) removing the constraint that SCU extraction be exhaustively; (ii) eliminating the difficult task of merging duplicate SCUs from different reference summaries; and (iii) sampling from the set of SCUs instead of explicitly assigning importance weights. They divide the process into two AMT tasks: (i) Pyramid creation, in which SCUs are obtained from reference summaries, and (ii) System summary evaluation using the created SCUs. The final score of a system summary is the percentage of SCUs that it matched.



==> representative_systems.tex <==
\subsection{Representative Systems} \label{sec:system}
% \pg{we want to make a table of these with some properties. For now we are just listing them.}
% \pfliu{Make sense!}
% \pfliu{Should we also do some experiments based on extractive summarization systems? }

% systems with state-of-the-art performance or the top performace on benchmark datasets

We use the following representative top-scoring systems that either achieve state-of-the-art (SOTA) results or competitive performance, for which we could gather the outputs on the \texttt{CNNDM} dataset.
%\footnote{We contacted the authors of these systems to gather the corresponding outputs. We also gather outputs of differet model variants.} 
%\gn{Try to put footnotes after punctuation.}

% \subsection{Extractive Summarizers} 
% \pfliu{Hi, Manik, Probably you can try to list names of our collected ext-summarizers. Then, we can decide if we need more.}
\paragraph{Extractive summarization systems.}
% Generally,  most of the existing extractive summarization systems follow a framework consisting of three major modules: \textit{sentence encoder}, \textit{document encoder} and \textit{decoder}.
% In this paper, we consider the outputs from extractive summarizers with different choices of encoders and decoders. 
% \gn{when you have a big list like this it is usually nice to have them in some coherent order, for example chronological order, alphabetical order, or order of performance.}
We use  
CNN-LSTM-BiClassifier (CLSTM-SL; \citet{kedzie2018content}),
Latent~\cite{zhang-etal-2018-neural-latent},
BanditSum~\cite{dong-etal-2018-banditsum}, 
REFRESH~\cite{narayan-etal-2018-ranking},
HIBERT ~\cite{zhang-etal-2019-hibert},
Bert-Sum-Ext~\cite{liu-lapata-2019-text},
CNN-Transformer-BiClassifier (CTrans-SL; \citet{zhong2019searching}), 
CNN-Transformer-Pointer (CTrans-PN; \citet{zhong2019searching}),
HeterGraph~\cite{wang2020heterogeneous} and MatchSum~\cite{zhong2020extractive} 
as representatives of extractive systems. In total, we use 10 extractive system outputs for each document in the \texttt{CNNDM} test set. 
% \mb{We actually collect 15 but use 10 for human evals. Is saying 10 fine here?} 
%\gn{Could change ``collect'' to ``use''.}

% Additionally, we use a genetic algorithm~\cite{peyrard_genetic} which can simulate current and future extractive systems by generating summaries from the full scoring range~\cite{peyrard-2019-studying}. We optimize the algorithm to maximize each of the 5 evaluation metrics under study (section~\ref{sec:metrics}) to generate 500 extractive summaries, per document. After removing duplicates, we are left with \mb{XXX} summaries per document.

% We detail them below.

% \paragraph{MatchSum}~\cite{zhong2020extractive}

% \paragraph{HeterGraph}~\cite{wang2020heterogeneous}

% \paragraph{Bert-Sum-Ext}~\cite{liu-lapata-2019-text}

% \paragraph{CNN-LSTM-BiClassifier(CLSTM-SL)}\cite{kedzie2018content} 
% This summarizer adopts convolutional neural network as sentence encoder and LSTM to model the cross-sentence relation. Finally, each sentence will be scored by a binary classifier.

% \paragraph{CNN-Transformer-BiClassifier(CTrans-SL)}
% \cite{zhong2019searching}
% The document encoder in the above model is replaced with the Transformer layer.

% \paragraph{CNN-Transformer-Pointer(CTrans-PN)} \cite{zhong2019searching}
% The decoder is replaced with a pointer network to avoid the repetition.



% \subsection{Abstractive Summarizers}
% \pfliu{I just list some systems we have collected, feel free to complete, correct, re-name, or detail them. If needed, we can also organize all systems (ext and abs) in a table and using `$\checkmark$' and `$\times$' in different columns to characterize them.}

\paragraph{Abstractive summarization systems.}
% paraphrase the corpus and can use novel words. 
% The current abstractive summarization systems mainly focus on the \textit{encoder-decoder} paradigm.
We user pointer-generator+coverage \cite{see-etal-2017-get}, 
fastAbsRL \cite{chen-bansal-2018-fast-abs}, 
fastAbsRL-rank \cite{chen-bansal-2018-fast-abs}, 
Bottom-up \cite{gehrmann2018bottom}, 
NeuSum \cite{zhou-etal-2018-neural}, 
T5 \cite{raffel2019exploring-t5}, 
Unilm-v1 \cite{dong2019unified}, 
Unilm-v2 \cite{dong2019unified}, 
twoStageRL \cite{zhang2019pretraining}, 
preSummAbs \cite{liu2019text-presumm},
preSummAbs-ext \cite{liu2019text-presumm} 
BART \cite{lewis2019bart} and
Semsim \cite{yoon2020learning}
as abstractive systems. In total, we use 15 abstractive system outputs for each document in the CNNDM test set. 
% \mb{We actually collect 25 but use 15 for human evals} \\

% \noindent
% Overall, we take these 25 top-performing system outputs per document on the \texttt{CNNDM} test set and partition them into three parts:
% \begin{itemize}
%     \item \texttt{CNNDM Abs} denotes collected output summaries from abstractive systems.
%     \item \texttt{CNNDM Ext} denotes collected output summaries from extractive systems.
%     \item \texttt{CNNDM Mix} is the union of the two.
% \end{itemize}

% \paragraph{Seq2seq+coverage+pointer} \cite{see2017get}
% The model is built based on a sequence to sequence framework, the encoder and decoder of which are a single-layer bidirectional LSTM and a single-layer unidirectional LSTM with copy and coverage mechanism.



%. It is capable of copying words in source document through pointer mechanism as well as generating novel words.
%Moreover, it merges the coverage vector in input of decoder and adds the coverage loss to prevent repetition. 


% \textbf{\textit{Seq2Seq-Coverage-Copy(S2S-Co-PN)}} \cite{see2017get}
% \paragraph{Seq2seq+coverage+pointer} \cite{see2017get}
% The model is built based on a sequence to sequence framework, the encoder and decoder of which are a single-layer bidirectional LSTM and a single-layer unidirectional LSTM with copy and coverage mechanism.

% \paragraph{Seq2seq+coverage}
% \paragraph{Seq2seq}
% %. It is capable of copying words in source document through pointer mechanism as well as generating novel words.
% %Moreover, it merges the coverage vector in input of decoder and adds the coverage loss to prevent repetition. 
% \paragraph{T5}
% \paragraph{BART}
% \paragraph{Bottom-up}
% \paragraph{NeuSum}
% \paragraph{Unilm-v1}
% \paragraph{Unilm-v2}
% \paragraph{fastAbsRL}
% \paragraph{fastAbsRL-rank}
% \paragraph{Semsim}
% \paragraph{twoStageRL}
% \paragraph{preSummAbs}
% \paragraph{preSummAbs-ext}

